Regular partitions of gentle graphs

Szemeredi's Regularity Lemma is a very useful tool of extremal combinatorics. Recently, several refinements of this seminal result were obtained for special, more structured classes of graphs. We survey these results in their rich combinatorial context. In particular, we stress the link to the theory of (structural) sparsity, which leads to alternative proofs, refinements and solutions of open problems. It is interesting to note that many of these classes present challenging problems. Nevertheless, from the point of view of regularity lemma type statements, they appear as "gentle" classes.

==> definitions.tex <==

\section{Order-defined classes: simpler semi-algebraic classes}
We call a class $\mathscr C$ {\em order-defined} if it is included in
the age of a graph definable in $(\mathbb Q,<)$, the countable dense
linear order without endpoints.  It is immediate that order-defined
classes are semi-algebraic.

\begin{example}
  The class of circle graphs is order-defined. It follows that the
  class of cographs, and more generally the class of permutation
  graphs and the class of distance-hereditary graphs (which are both
  contained in the class of circle graphs) are order-defined.
\end{example}

However, we are not aware of any example of a semi-algebraic class that is provably not order-defined.

The notion of order-defined classes is very similar to the notion of Boolean dimension considered by Gambosi, Ne\v set\v ril, and Talamo \cite{GAMBOSI1990251} and by Ne\v set\v ril and Pudl\'ak \cite{Nesetril1989}. The {\em Boolean dimension} of a poset $P=(X,\leq)$ is the minimum number of linear orders on $X$ a Boolean combination of which gives $\leq$. Thus we have the following property:
\begin{observation}
	If a class $\mathcal P$ of posets has bounded Boolean dimension then the class of the comparability graphs of the posets in $\mathcal P$ is order-defined.
\end{observation}

The conjecture on boundedness of Ne\v set\v ril and Pudl\'ak \cite{Nesetril1989} on the boundedness of the Boolean dimension of planar posets can thus be weakened as follows.
\begin{conjecture}
	The class of comparability graphs of planar posets is order-defined.
\end{conjecture}


==> rw.tex <==
\section{Regularity for classes $2$-covered by a class with bounded rankwidth}
\label{sec:rw}
In this section, we extend our study from embedded $m$-partite cographs. In particular, we extend \Cref{lem:empc_order} to classes with bounded rankwidth (\Cref{lem:rw}) and deduce that every class 
$2$-covered by a class with bounded rankwidth is order-defined, hence satisfy the regularity lemma for semi-algebraic classes (\Cref{cor:rw-2cov-reg}). However, in this setting, we do not have the explicit construction nor the explicit bounds we were able to provide in \Cref{cor:reg_emb_2cov} and \Cref{cor:reg_emb_2cov_equi}.
Note that there are indeed classes of graphs that are $2$-covered by a class with bounded rankwidth and not by a class of embedded $m$-partite cographs. In particular, the class of graphs with rankwidth at most $3$, being not linearly $\chi$-bounded (see e.g.~\cite{msrw}), is not covered by a class of embedded $m$-partite cographs ,though it is trivially $2$-covered by a class with bounded rankwidth.

\begin{lemma}
\label{lem:rw1}
Let $G$ be a graph with rankwidth at most $r$. Then there exist~$r$
graphs $G_1,\dots,G_r$ with vertex set $V(G)$ and edge sets
$E_1,\dots,E_r$, such that:
\begin{enumerate}
\item each $G_i$ has rankwidth at most $1$,
\item $E=\bigoplus_{i=1}^r E_i$, where $E_i\bigoplus E_j$ denotes the
  symmetric difference of $E_i$ and~$E_j$.
\end{enumerate}
\end{lemma}
\begin{proof}
  We show the statement by induction on $|G|$. The statement is
  trivial for graphs with $|G|\leq 4$.  For $|G|\geq 5$, let
  $(V_1,V_2)$ be a vertex partition of $G$ such that $G[V_1]$ and
  $G[V_2]$ have rankwidth at most $r$ and the cut-rank of $(V_1,V_2)$
  is at most $r$.  By induction hypothesis there exist
  $G_1^1,\dots,G_r^1$ with vertex set $V_1$ and $G_1^2,\dots,G_r^2$
  with vertex set $V_2$ such that $E(G[V_1])=\bigoplus E_i^1$ and
  $E(G[V_2])=\bigoplus E_i^2$. Let $A_1,\dots,A_k$, $k\leq r$, be a
  basis for the neighborhoods in $V_2$ of vertices in~$V_1$. Then for
  every vertex $u\in V_1$ there are coefficients $a_i(u)\in GF_2$ such
  that $N(u)\cap V_2=\bigoplus a_i(u)A_i$. We define
  \[
  E_i:=E_i^1\cup E_i^2\cup \{\{u,v\}\in V_1\times V_2\mid
  a_i(u)=1\text{ and }v\in A_i\}.
  \]
  Then it is immediate that $E(G)=\bigoplus_i E_i$ and, as the
  cut-rank of $(V_1,V_2)$ for each~$E_i$ is at most one, the
  graphs $G_i=(V(G),E_i)$ have rankwidth at most~$1$.
\end{proof}
The following lemma, though simple, is quite useful.
\begin{lemma}
\label{lem:Bool}
	Let $\mathscr D$ be  a distal-defined (resp.\ semi-algebraic, order-defined, set-defined) class, let $p$ be an integer, and let $\mathscr C$ be a class of graphs such that there exists a Boolean function $\Phi$ such that for each graph $G\in \mathscr C$ there exists $E_1,\dots,E_p$ with $E(G)=\Phi(E_1,\dots,E_p)$ and the subgraph $G_i$ of $G$ with edge set $E_i$ belongs to~$\mathscr D$.
	Then the class $\mathscr C$ is also 
distal-defined (resp.\ semi-algebraic, order-defined, set-defined).
\end{lemma}
\begin{proof}
		Let $\mathbf U$ be a graph definable in a distal structure (resp.\ a semi-algebraic graph, a graph definable in $(\mathbb Q,<)$, a graph definable in $\mathbb N$) such that $\mathscr D\subseteq{\rm Age}(\mathbf U)$.
		We consider the graph $\mathbf H$ whose vertex set is the set of all tuples $\bar v\in V(\mathbf U)^{p}$ and whose edges are defined by the formula 
$\phi(\bar x,\bar y):=\Phi(E(x_1,y_1),\dots,E(x_p,y_p))$.
		Then it is easily checked that $\mathscr C$ is included in the age of $\mathbf H$, which (being definable in $\mathbf U$) is definable in a distal structure (resp.\ a semi-algebraic graph, a graph definable in $(\mathbb Q,<)$, a graph definable in $\mathbb N$).
\end{proof}



\begin{lemma}
\label{lem:rw}
Classes with bounded rankwidth are order-defined.
\end{lemma}
\begin{proof}
  According to \Cref{lem:Bool} and \Cref{lem:rw1} it is sufficient to
  prove the result for the class of graphs with rankwidth at most $1$,
  that is for distance-hereditary graphs~\cite{OUM200579}. As
  distance-hereditary graphs are circle graphs they are order-defined.
\end{proof}


\begin{corollary}
  Every class $\mathscr C$ $2$-covered by a class with bounded
  rankwidth is order-defined.
\end{corollary}
\begin{proof}
  This theorem is a direct consequence of \Cref{lem:rw} and
  \Cref{thm:2cov}.
\end{proof}

The next corollary then follows from \Cref{thm:sa}, as every order-defined class is semi-algebraic.

\begin{corollary}
\label{cor:rw-2cov-reg}
	Let $\mathscr C$ be a class $2$-covered by a class with bounded
  rankwidth.
  %
	Then there exists a constant $c$ such
   that for every $0<\epsilon<1/2$ and every  $G\in\mathscr C$
there is an equipartition
   $V_1,\ldots, V_k$ of the vertex set into~$k$ classes with
   $k\leq (1/\epsilon)^c$ such that all but at most $\epsilon k^2$
   pairs are homogeneous.
\end{corollary}


